FedYolo: Augmenting Federated Learning with Pretrained Transformers

The growth and diversity of machine learning applications motivate a rethinking of learning with mobile and edge devices. How can we address diverse client goals and learn with scarce heterogeneous data? While federated learning aims to address these issues, it has challenges hindering a unified solution. Large transformer models have been shown to work across a variety of tasks achieving remarkable few-shot adaptation. This raises the question: Can clients use a single general-purpose model, rather than custom models for each task, while obeying device and network constraints? In this work, we investigate pretrained transformers (PTF) to achieve these on-device learning goals and thoroughly explore the roles of model size and modularity, where the latter refers to adaptation through modules such as prompts or adapters. Focusing on federated learning, we demonstrate that: (1) Larger scale shrinks the accuracy gaps between alternative approaches and improves heterogeneity robustness. Scale allows clients to run more local SGD epochs which can significantly reduce the number of communication rounds. At the extreme, clients can achieve respectable accuracy locally highlighting the potential of fully-local learning. (2) Modularity, by design, enables $>$100$\times$ less communication in bits. Surprisingly, it also boosts the generalization capability of local adaptation methods and the robustness of smaller PTFs. Finally, it enables clients to solve multiple unrelated tasks simultaneously using a single PTF, whereas full updates are prone to catastrophic forgetting. These insights on scale and modularity motivate a new federated learning approach we call "You Only Load Once" (FedYolo): The clients load a full PTF model once and all future updates are accomplished through communication-efficient modules with limited catastrophic-forgetting, where each task is assigned to its own module.

==> sec/local_fed.tex <==
\begin{figure}\label{fig:localfed_homo}
\centering
%\hspace{-35pt}
\begin{subfigure}{1.7in}
    \centering
	\begin{tikzpicture}
		\node at (0,0) [scale=0.29]{\includegraphics{img/cifar10_module_fedlocal.pdf}};
		\node at (-2.3 ,0) [scale=0.8,rotate=90] {Accuracy};
		\node at (0,-1.9) [scale=0.8] {\# of samples};
	\end{tikzpicture}\vspace{-4pt}\caption{Homogeneous, Module, Cifar10}\label{fig:localfed_homo_1}
\end{subfigure}
\begin{subfigure}{1.7in}
    \centering
	\begin{tikzpicture}
		\node at (0,0) [scale=0.29]{\includegraphics{img/cifar100_module_fedlocal_new.pdf}};
		\node at (-2.3 ,0) [scale=0.8,rotate=90] {Accuracy};
		\node at (0,-1.9) [scale=0.8] {\# of samples};
	\end{tikzpicture}\vspace{-4pt}\caption{Homogeneous, Module, Cifar100}\label{fig:localfed_homo_2}
\end{subfigure}\\
% \begin{subfigure}{1.7in}
%     \centering
% 	\begin{tikzpicture}
% 		\node at (0,0) [scale=0.29]{\includegraphics{img/Not_ready.png}};
% 		\node at (-2.3 ,0) [scale=0.8,rotate=90] {Accuracy};
% 		\node at (0,-1.9) [scale=0.8] {\# of samples};
% 	\end{tikzpicture}\vspace{-4pt}\caption{Homo,Module, FEMNIST}\label{fig:localfed_homo_3}
% \end{subfigure}\\
\begin{subfigure}{1.7in}
    \centering
	\begin{tikzpicture}
		\node at (0,0) [scale=0.29]{\includegraphics{img/cifar10_module_fedlocal.pdf}};
		\node at (-2.3 ,0) [scale=0.8,rotate=90] {Accuracy};
		\node at (0,-1.9) [scale=0.8] {\# of samples};
	\end{tikzpicture}\vspace{-4pt}\caption{Homogeneous, Fully, Cifar10}\label{fig:localfed_homo_4}
\end{subfigure}
\begin{subfigure}{1.7in}
    \centering
	\begin{tikzpicture}
		\node at (0,0) [scale=0.29]{\includegraphics{img/cifar100_fully_fedlocal_new.pdf}};
		\node at (-2.3 ,0) [scale=0.8,rotate=90] {Accuracy};
		\node at (0,-1.9) [scale=0.8] {\# of samples};
	\end{tikzpicture}\vspace{-4pt}\caption{Homogeneous, Fully, Cifar100}\label{fig:localfed_homo_5}
\end{subfigure}
% \begin{subfigure}{1.7in}
%     \centering
% 	\begin{tikzpicture}
% 		\node at (0,0) [scale=0.29]{\includegraphics{img/Not_ready.png}};
% 		\node at (-2.3 ,0) [scale=0.8,rotate=90] {Accuracy};
% 		\node at (0,-1.9) [scale=0.8] {\# of samples};
% 	\end{tikzpicture}\vspace{-4pt}\caption{Homo,Fully, FEMNIST}\label{fig:localfed_homo_6}
% \end{subfigure}
\caption{Homogeneous,Solid: fully local, dashed: fed. Rows: Module vs full federated. Columns: dataset. 2x2 dimensions: (local, federated) x (module, full). Main message: fully local vs federated in a single figure.}
\label{fig:localfed_homo}
\end{figure}

% \begin{figure}
% \centering
% %\hspace{-35pt}
% \begin{subfigure}{1.7in}
%     \centering
% 	\begin{tikzpicture}
% 		\node at (0,0) [scale=0.29]{\includegraphics{img/Not_ready.png}};
% 		\node at (-2.3 ,0) [scale=0.8,rotate=90] {Accuracy};
% 		\node at (0,-1.9) [scale=0.8] {\# of samples};
% 	\end{tikzpicture}\vspace{-4pt}\caption{Heterogeneous,Module, Cifar10}\label{fig:localfed_heter_1}
% \end{subfigure}
% \begin{subfigure}{1.7in}
%     \centering
% 	\begin{tikzpicture}
% 		\node at (0,0) [scale=0.29]{\includegraphics{img/Not_ready.png}};
% 		\node at (-2.3 ,0) [scale=0.8,rotate=90] {Accuracy};
% 		\node at (0,-1.9) [scale=0.8] {\# of samples};
% 	\end{tikzpicture}\vspace{-4pt}\caption{Heterogeneous,Module, Cifar100}\label{fig:localfed_heter_2}
% \end{subfigure}
% \begin{subfigure}{1.7in}
%     \centering
% 	\begin{tikzpicture}
% 		\node at (0,0) [scale=0.29]{\includegraphics{img/Not_ready.png}};
% 		\node at (-2.3 ,0) [scale=0.8,rotate=90] {Accuracy};
% 		\node at (0,-1.9) [scale=0.8] {\# of samples};
% 	\end{tikzpicture}\vspace{-4pt}\caption{Heterogeneous,Module, FEMNIST}\label{fig:localfed_heter_3}
% \end{subfigure}\\
% \begin{subfigure}{1.7in}
%     \centering
% 	\begin{tikzpicture}
% 		\node at (0,0) [scale=0.29]{\includegraphics{img/Not_ready.png}};
% 		\node at (-2.3 ,0) [scale=0.8,rotate=90] {Accuracy};
% 		\node at (0,-1.9) [scale=0.8] {\# of samples};
% 	\end{tikzpicture}\vspace{-4pt}\caption{Heterogeneous,Fully, Cifar10}\label{fig:localfed_heter_4}
% \end{subfigure}
% \begin{subfigure}{1.7in}
%     \centering
% 	\begin{tikzpicture}
% 		\node at (0,0) [scale=0.29]{\includegraphics{img/Not_ready.png}};
% 		\node at (-2.3 ,0) [scale=0.8,rotate=90] {Accuracy};
% 		\node at (0,-1.9) [scale=0.8] {\# of samples};
% 	\end{tikzpicture}\vspace{-4pt}\caption{Heterogeneous,Fully, Cifar100}\label{fig:localfed_heter_5}
% \end{subfigure}
% \begin{subfigure}{1.7in}
%     \centering
% 	\begin{tikzpicture}
% 		\node at (0,0) [scale=0.29]{\includegraphics{img/Not_ready.png}};
% 		\node at (-2.3 ,0) [scale=0.8,rotate=90] {Accuracy};
% 		\node at (0,-1.9) [scale=0.8] {\# of samples};
% 	\end{tikzpicture}\vspace{-4pt}\caption{Heterogeneous,Fully, FEMNIST}\label{fig:localfed_heter_6}
% \end{subfigure}
% \caption{Heter,Solid: fully local, dashed: fed}
% \label{fig:localfed_heter}
% \end{figure}


==> sec/sanity_check.tex <==
\section{Ablation experiments}
\subsection{}
\begin{figure}
\centering
%\hspace{-35pt}
% \begin{subfigure}{1.7in}
%     \centering
% 	\begin{tikzpicture}
% 		\node at (0,0) [scale=0.29]{\includegraphics{img/prompt_length.png}};
% \end{tikzpicture}\vspace{-4pt}\caption{In \cite{lester2021power}}\label{fig:comm_1_1}
% \end{subfigure}
\begin{subfigure}{1.7in}
    \centering
	\begin{tikzpicture}
		\node at (0,0) [scale=0.29]{\includegraphics{img/cifar100_num_para.pdf}};
\end{tikzpicture}\vspace{-4pt}\caption{}\label{fig:comm_1_2}
\end{subfigure}
\caption{In \cite{lester2021power}, the results indicate that there is a saturation point of prompt size in performance improvement. Beyond that value, further increasing the prompt size does not lead to a significant improvement in performance. Our results also verify the same conclusion. }
\label{fig:comm}
\end{figure}

==> sec/todo.tex <==
\section*{Basic TODOs}

\textbf{Framing:} This is an exhaustive study on vision transformers and federated learning. We explore all axes. While some results are as expected and some are less obvious.



Naming convention:
\begin{itemize}
% \item Full update($\fullup$) vs Modular update($\modular$)
% %\item Personal, Personalized FL, FL
% \item Local-only Learning($\local$), FedAvg($\FedAvg$), FedAvg+Local($\Fedlocal$)
\item Full update vs Modular update
%\item Personal, Personalized FL, FL
\item Local-only Learning, FedAvg, FedAvg+Local
\end{itemize}
Give names to the core findings in the intro to set the stage and keep consistency throughout

Interesting axes:
\begin{itemize}
 \item  Personalization approaches -- Less need for personalization at scale
 \begin{itemize}
 \item Bring up exciting aspects of personalized
 \end{itemize}
 \item  Robustness to hetero of scale
 \item  Non-forgetting ability of scale
 \item  Multitasking
 \item  Few-shot efficiency modules -- Module gap closes eventually
\end{itemize}
Not-as-interesting axes:
\begin{itemize}
\item Communication
\item Accuracy benefit of scale
\end{itemize}


\xuechen{Samet, Xuechen?}
\begin{itemize}
    \item homogeneous
    \begin{itemize}
        \item fully finetune v.s. module
        \item federated training v.s. fully local
    \end{itemize}
    \item heterogeneous
    \begin{itemize}
        \item robustness
        \item personalize: personalize v.s. fully local
        \item forgetting
        \item allow larger local epoch
    \end{itemize}
    \item multi-task
    \item efficiency (communication cost)
    \begin{itemize}
        \item module help
        \item scale, with larger local epoch
    \end{itemize}
\end{itemize}

==> sec/zz_intro.tex <==
\section{Introduction}
\label{sect introduction}





% We aim to answer the following questions:
% \begin{itemize}
%     \item Large model can achieve
%     \begin{itemize}
%         \item Better few-shot, good fully-local acc (avoid federated)
%         \begin{itemize}
%             \item Personalization vs fully-local (what class distribution?)
%         \end{itemize}
%         \item Fewer rounds, more local epoch
%         \item Overfitting benefit of module for personalization
%     \end{itemize}
%     \item Prompt-tuning is more robust to hetero than fine-tuning 
%     \item Prompt-tuning is comm efficient
%     \begin{itemize}
%         \item No forgetting
%     \end{itemize}
% \end{itemize}

% \xuechen{New structure?}

% List of experiments:
% \begin{itemize}
%     \item federated learning across all clients --> evaluate on all 100 classes
%     \item local learning across all clients ---> evaluate on all 100 classes
%       \item federated learning + local learning across all clients --> evaluate on all 100 classes
%      \item federated learning across all clients --> evaluate on local 20 classes (same as bullet 1)
%     \item local learning across all clients ---> evaluate on local 20 classes
%       \item federated learning + local learning across all clients --> evaluate on local 20 classes
% \end{itemize}

%Since its inception, federated learning (FL) has enjoyed significant success as a collaborative machine learning paradigm for decentralized clients. On the other hand, there are several overarching challenges

The landscape of machine learning applications has seen a dramatic evolution in recent years. Far surpassing the conventional tasks in computer vision and natural language processing, state-of-the-art machine learning (ML) models display exceptional competencies in generative modeling, including image, text, and code, as well as in multimodal learning and decision making. Propelling these advancements are architectural innovations, in particular the advent of transformers, and the growing trend of retraining these models on vast datasets. As these advances make their way into mobile and edge devices, they also motivate a fundamental rethinking of contemporary federated learning (FL) approaches. Notably, pretrained transformers (PTF) can be few-shot \emph{adapted} to a wide range of downstream tasks, and for this reason, large PTFs are often referred to as foundation models~\cite{bommasani2021opportunities}. Intuitively, this capability will boost the data efficiency of federated learning and provide a flexible platform for addressing the diverse needs of mobile clients, which is the focus of this paper. 
Rather than requiring multiple custom models for individual tasks, we explore whether clients can instead deploy a few PTF models with multitask capabilities. \amit{Agree with Jiasi. We should say a little more on scale and comms, and then say that this enables multi-tasking, like in the abstract.}
\jiasi{to discuss: is multitask the main focus, or should we bring in first scale and communication aspects before that?}
While this idea is simple conceptually, can we actually realize such benefits in a practical federated learning setting with heterogeneous client data and communication bottlenecks? More generally, what are the right practices and algorithms for federated learning with PTFs? 

Towards providing concrete answers to such questions, this work thoroughly explores federated learning with PTFs and focuses on two central considerations as follows.
\textbf{(A) Scale:} PTFs enjoy substantial benefits from larger model sizes~\cite{lester2021power} -- as well as more computation and data during pretraining. 
The question is: in a federated setting, do clients also benefit from the power of scale?
\textbf{(B) Modularity:} PTFs can be adapted to a wide range of downstream tasks through parameter-efficient modules such as prompt- or adapter-tuning. The question is: in a federated setting, how should client utilize these modules?
Modularity naturally suggests a PTF-specific FL strategy that we call \emph{modular updates}: Clients keep their PTF frozen throughout the training, and only train and communicate modules (and a classifier head) to adapt their PTFs to a new task. This is in contrast to conventional \emph{full-parameter updates} where clients send/receive all parameters of the model.

To explore this, we consider an FL setting where clients have heterogeneous/non-IID data that might stem from multiple distinct learning tasks (e.g.~text vs object recognition). We study three training schemes, each of which can be implemented in a modular- or full-update fashion: In \local, each client trains its model using its private data. \FedAvg is the standard federated learning averaging scheme. Finally, \Fedlocal is a simple personalization scheme where clients locally fine-tune following $\FedAvg$. \amit{An immediate question from reviewers can be why are we looking at FedAvg and its variants, rather than newer methods? We should proactively address this. Is it that the existing methods with FL + transformers use FedAvg+. If so, we can just say "sota methods" and cite.} The training strategies we explore are depicted in Figure \ref{main_fig}. In a nutshell, our main message is that \emph{large PTFs with modular updates enable communication-efficient, robust, and multitask FL}. This message generalizes well across different module choices (prompt, LoRA, adapter) pointing to a universal benefit of parameter-efficient FL with large models. Specifically, we make the following contributions:

%\begin{itemize}
$\bullet$ \textbf{Scale.} Scale reduces the reliance on personalization and collaboration by shrinking the accuracy gaps between \FedAvg and \Fedlocal as well as \Fedlocal and \local. On the other hand, modular update performs on par with full update when the scale is large and it often outperforms under few-shot/scarce data.\xuechen{few-shot or hetero} This makes modular update a more viable strategy for \local and  via \Fedlocal. \jiasi{message not clear -- what is expected and what is unexpected? Jiasi will revisit later}

$\bullet$ \textbf{Heterogeneity.} Scale boosts robustness to heterogeneous client \jiasi{data? class?} distributions, while the modularity particularly helps the robustness of smaller PTFs. They also provide resilience to forgetting: \Fedlocal accuracy remains competitive with \FedAvg on the global distribution even after the local-learning phase. \amit{Is there an intuition behind why forgetting is mitigated?} \jiasi{agree with Amit's comment -- what is intuition/expected/unexpected? Jiasi will revisit. SO: We can cite this paper \cite{tripuraneni2021overparameterization}. Not sure if there is an earlier federated paper with same finding.}

$\bullet$ \textbf{Communication.} Large PTFs can potentially contain billions of parameters whereas the module size is often in the order of millions. Thus intuitively, updating only the modules can save significantly on communication costs. We find that such modular update unlocks orders-of-magnitude communication savings compared to full update while maintaining, and often accelerating, the rate of convergence in number of communication rounds. 

\begin{wrapfigure}{r}{6.5cm}
\vspace{-0.55cm}
\centering
\includegraphics[scale=0.5]{img/fedyolo2.pdf}
        \vspace{-10pt}
\caption{\small{\yolo: Multitask FL with pretrained transformers: Clients download the PTF when training starts. All future updates are through parameter-efficient modules. Each task is assigned a unique module. Clients can further personalize the modules.}}
\vspace{-10pt}
\label{fig:yolo}%\vspace{-30pt}
\end{wrapfigure}
$\bullet$ \textbf{Multitask learning.} In a multitask setting where FL clients collaboratively and simultaneously learn multiple disparate tasks (e.g., classification on different domains such as the CIFAR, CelebA, and FEMNIST datasets), the challenge is determining which parts of the model to update. We propose a \yolo algorithm that assigns isolated modules to each task while keeping a single PTF (see Figure \ref{fig:yolo}). \amit{These are datasets, not tasks. The tasks may be different, but we need to clarify. They all do recognition, which is the same task.}
We demonstrate that \yolo incurs minimal, if any, performance degradation compared to learning each task in isolation. %, whereas a standard \FedAvg scheme with full update is prone to failure as the number of tasks grows. 
%For instance, Figure \ref{fig:multitask} shows that in a setting with four learning tasks, with \fullup, performance of $\Fedlocal$ is not even distinguishable from $\local$ whereas \yolo substantially outperforms both.
%\smallskip

%\end{itemize}
%representation conflicts and forgetting 
Our findings have important implications. Adapting the PTFs via modular update not only provides a simple communication-efficient strategy with relatively minor drawbacks but also significant potential upside in terms of personalization, robustness, and multitasking. For instance, we show that combined benefits of modular update and larger scale makes \local a fairly competitive alternative to FL approaches \FedAvg or \Fedlocal, hinting at the viability of perfect-privacy (by sidestepping FL). Additionally, our proposal \yolo (stands for ``You Only (Down)Load Once'') enables the clients to use a single PTF and multiple small modules to address diverse set of mobile ML goals, avoiding the need for maintaining/training multiple models.

%\smallskip
%\xuechen{hope to add, the challenge in federated learning: For example: why closing the gap between fed v.s. local is pretty important. Privacy. e.g. patient data}
%\chang{ Initial version.}
























\begin{comment}
In this paper, we first show that many properties of transformers improve as the scale of the model increases. To deploy large transformer models in scenarios involving mobile applications, such as federated learning (FL), we aim to avoid training large-scale transformers from scratch or conducting full fine-tuning on all parameters. In light of this, we investigate whether these properties still hold when performing parameter-efficient fine-tuning on a limited number of parameters in pre-trained transformers.

If our empirical findings demonstrate that parameter-efficient tuning methods, such as Low-Rank Adaptation (LoRA \cite{hu2021lora}), Visual Prompt Tuning (VPT\cite{jia2022visual}), and Adapter\cite{houlsby2019parameterefficient}, exhibit similar performance to fully fine-tuned transformers, it would significantly contribute to the applicability of vision transformers in mobile/edge device environments.

To achieve this goal, our study is organized as follows:

We provide a comprehensive analysis of the improvements in various properties of transformers as the scale of the model increases. This analysis establishes a foundation for our subsequent investigations into the efficacy of parameter-efficient fine-tuning methods.

We conduct extensive experiments to compare the performance of parameter-efficient tuning methods, with fully fine-tuned transformers. Our experimental results will reveal whether these techniques can maintain the advantages of large-scale transformers while reducing the computational and communication overhead.

We discuss the implications of our findings for the deployment of vision transformers in mobile applications, particularly in the context of federated learning. By demonstrating the effectiveness of parameter-efficient fine-tuning methods, our work could potentially pave the way for more widespread adoption of vision transformers in resource-constrained environments.

In conclusion, our study aims to provide valuable insights into the properties of large-scale transformers and the potential of parameter-efficient fine-tuning methods. By confirming the effectiveness of these techniques, we hope to facilitate the deployment of vision transformers in mobile applications, ultimately enhancing their real-world applicability and utility.
\end{comment}
